Effect of halogen dopants on the Li$_{2}$O$_{2}$ properties: Is chloride special?

There is consensus on the fact that one of the main limitations of the Li air batteries (LABs) is the insulating character of Li$_{2}$O$_{2}$ and that it becomes crucial to explore new conduction paths. Recent studies indicate that doping with chloride increases the ion conductivity of Li$_{2}$O$_{2}$, although to a much lesser extent than expected if chloride is assumed as a donor dopant [Gerbig et al., Adv. Mater.,2013, 25, 3129]. Subsequently, it has been shown that the addition of lithium chloride, LiCl, to the battery electrolyte increases its discharge capacity while this effect is not observed with other halogens [Matsuda et al., J. Phys. Chem. C, 2016, 120, 13360]. This fact was attributed to an increase in the conductivity of Cl-doped Li$_{2}$O$_{2}$, but still the responsible mechanism is not clear. In this work, we have performed first principle calculations to study the effect of the different halogens (F, Cl, Br, I) as substitutional defects in the electronic and transport properties of Li$_{2}$O$_{2}$. We have calculated the formation energies of the different defects and impurities and we analysed how they affect the activation barriers and diffusion coefficients . We have demonstrated that the chloride does not behave like a donor dopant, thus explaining the meager increase of the ionic conductivity experimentally observed neither it promotes the polaron formation and its mobility. We have also found that chloride does not present any special behaviour among the halogen series. Our results reveal that all the studied configurations associated with the halogen defects do not derive in metallic states nor extra polarons that would increase considerably the electronic conductivity. This is mainly due to the ionic characteristics of the Li$_{2}$O$_{2}$ crystal and the capability of the oxygen dimers to adapt its valence rather than to the nature of the dopant itself.

==> salida <==
4c4,5
< journal={The Journal of Chemical Physics},
---
> title={Hybrid functionals based on a screened Coulomb potential},
> journal={J. Chem. Phys.},
7c8
< pages={8207},
---
> pages={8207--8215},
8a10
> doi = {10.1063/1.1564060},
15c17
<  journal = {The Journal of Chemical Physics},
---
>  journal = {J. Chem. Phys.},
18c20
<  pages = {219906},
---
>  pages = {219906--219906},
59c61
< journal = {The Journal of Physical Chemistry C},
---
> journal = {J. Phys. Chem. C},
62c64
< pages = {5568-5577},
---
> pages = {5568--5577},
70c72
< journal = {The Journal of Chemical Physics},
---
> journal = {J. Chem. Phys.},
79c81
< author = { Kresse, G. and Furthmuller, J.},
---
> author = {Kresse, G. and Furthmuller, J.},
83c85
< pages = {15},
---
> pages = {15--50},
84a87
> doi={10.1016/0927-0256(96)00008-0},
93c96
< pages = {11169},
---
> pages = {11169--11186},
94a98
> doi={10.1103/PhysRevB.54.11169},
102a107
> pages = {B864--B870},
108c113
< journal = {The Journal of Chemical Physics},
---
> journal = {J. Chem. Phys.},
119c124
< journal = {Advanced Materials},
---
> journal = {Adv. Mater.},
122,124d126
< publisher = {WILEY-VCH Verlag},
< issn = {1521-4095},
< url = {http://dx.doi.org/10.1002/adma.201300264},
127d128
< keywords = {alkali peroxides, defect chemistry, electrochemistry, Li-batteries},
134c135
< journal = {Chemistry of Materials},
---
> journal = {Chem. Mater.},
137c138
< pages = {2952-2959},
---
> pages = {2952--2959},
171c172
< journal = {The Journal of Physical Chemistry C},
---
> journal = {J. Phy. Chem. C},
174c175
< pages = {25222-25228},
---
> pages = {25222--25228},
182c183
< journal = {Chemistry of Materials},
---
> journal = {Chem. Mater.},
185c186
< pages = {839-847},
---
> pages = {839--847},
206c207
< journal = {The Journal of Physical Chemistry C},
---
> journal = {J. Phys. Chem. C},
217c218
< journal = {Journal of Power Sources},
---
> journal = {J. Power Sources},
226c227
< journal = {Applied Physics Letters},
---
> journal = {Appl. Phys. Lett.},
237c238
< journal = {Journal of the American Chemical Society},
---
> journal = {J. Am. Chem. Soc.},
240c241
< pages = {1093-1103},
---
> pages = {1093--1103},
243d243
< note ={PMID: 22148314},
255d254
< publisher = {American Physical Society},
262c261
< journal = {Chemical Reviews},
---
> journal = {Chem. Rev.},
268d266
< note ={PMID: 25376975},
289c287
< pages = {A1133--A1138},
---
> pages = {1133--1138},
299c297
< journal = {Chemistry of Materials},
---
> journal = {Chem. Mater.},
302c300
< pages = {8406},
---
> pages = {8406--8413},
314c312
< pages  ={2370},
---
> pages  ={2370--2379},
325c323
< pages = {B864--B871},
---
> pages = {864--871},
355a354
>   title={Advances in understanding mechanisms underpinning lithium–air batteries},
357c356
<   journal = {Nature Energy},
---
>   journal = {Nat. Energy},
359c358
<   pages = {16128},
---
>   pages = {1--11},
360a360
>   doi = {10.1038/nenergy.2016.128},
373,374d372
<   month = {Jul},
<   publisher = {American Physical Society},
376d373
<   url = {https://link.aps.org/doi/10.1103/PhysRevB.86.045112}
382c379
<  journal = {Journal of Applied Physics},
---
>  journal = {J. Appl. Phys.},
385c382
<  pages = {3851-3879},
---
>  pages = {3851--3879},
398,399c395
< pages  ="1555-1563",
< publisher  ="The Royal Society of Chemistry",
---
> pages  ="1555--1563",
401,402c397
< url  ="http://dx.doi.org/10.1039/C3EE43870H",
< abstract  ="Researchers worldwide view the high theoretical specific energy of the lithium-air or lithium-oxygen battery as a promising path to a transformational energy-storage system for electric vehicles. Here{,} we present a self-consistent material-to-system analysis of the best-case mass{,} volume{,} and cost values for the nonaqueous lithium-oxygen battery and compare them with current and advanced lithium-based batteries using metal-oxide positive electrodes. Surprisingly{,} despite their high theoretical specific energy{,} lithium-oxygen systems were projected to achieve parity with other candidate chemistries as a result of the requirement to deliver and purify or to enclose the gaseous oxygen reactant. The theoretical specific energy{,} which leads to predictions of an order of magnitude improvement over a traditional lithium-ion battery{,} is shown to be an inadequate predictor of systems-level cost{,} volume{,} and mass. This analysis reveals the importance of system-level considerations and identifies the reversible lithium-metal negative electrode as a common{,} critical high-risk technology needed for batteries to reach long-term automotive objectives. Additionally{,} advanced lithium-ion technology was found to be a moderate risk pathway to achieve the majority of volume and cost reductions."}
---
> }
411,412c406
< pages  ="750-768",
< publisher  ="The Royal Society of Chemistry",
---
> pages  ="750--768",
414,415c408
< url  ="http://dx.doi.org/10.1039/C3EE23966G",
< abstract  ="Rechargeable energy storage systems with high energy density and round-trip efficiency are urgently needed to capture and deliver renewable energy for applications such as electric transportation. Lithium-air/lithium-oxygen (Li-O2) batteries have received extraordinary research attention recently owing to their potential to provide positive electrode gravimetric energies considerably higher ([similar]3 to 5[times]) than Li-ion positive electrodes{,} although the packaged device energy density advantage will be lower ([similar]2[times]). In light of the major technological challenges of Li-O2 batteries{,} we discuss current understanding developed in non-carbonate electrolytes of Li-O2 redox chemistry upon discharge and charge{,} oxygen reduction reaction product characteristics upon discharge{,} and the chemical instability of electrolytes and carbon commonly used in the oxygen electrode. We show that the kinetics of oxygen reduction reaction are influenced by catalysts at small discharge capacities (Li2O2 thickness less than [similar]1 nm){,} but not at large Li2O2 thicknesses{,} yielding insights into the governing processes during discharge. In addition{,} we discuss the characteristics of discharge products (mainly Li2O2) including morphological{,} electronic and surface features and parasitic reactivity with carbon. On charge{,} we examine the reaction mechanism of the oxygen evolution reaction from Li2O2 and the influence of catalysts on bulk Li2O2 decomposition. These analyses provide insights into major discrepancies regarding Li-O2 charge kinetics and the role of catalyst. In light of these findings{,} we highlight open questions and challenges in the Li-O2 field relevant to developing practical{,} reversible batteries that achieve the anticipated energy density advantage with a long cycle life."}
---
> }
427,428c420
< url  ="http://dx.doi.org/10.1039/C5CC04620C",
< abstract  ="The Li-air battery has received significant attention over the past decade given its high theoretical specific energy compared to competing energy storage technologies. Yet{,} numerous scientific challenges remain unsolved in the pursuit of attaining a battery with modest Coulombic efficiency and high capacity. In this Feature Article{,} we provide our current perspective on challenges facing the development of nonaqueous Li-O2 battery cathodes. We initially present a review on our understanding of electrochemical processes occurring at the nonaqueous Li-O2 cathode. Electrolyte and cathode instabilities and Li2O2 conductivity limitations are then discussed{,} and suggestions for future materials research development to alleviate these issues are provided."}
---
> }
433c425
< journal ="Nature Chemistry",
---
> journal ="Nature Chem.",
437,438c429,430
< pages={1091 },
< url={http://dx.doi.org/10.1038/nchem.2101}
---
> pages={1091--1099},
> doi={10.1038/nchem.2101},
441,457d432
< @article{TAN2017155,
< title = "Advances in modeling and simulation of Li air batteries",
< journal = "Progress in Energy and Combustion Science",
< volume = "62",
< number = "Supplement C",
< pages = "155 - 189",
< year = "2017",
< issn = "0360-1285",
< doi = "https://doi.org/10.1016/j.pecs.2017.06.001",
< url = "http://www.sciencedirect.com/science/article/pii/S0360128517300278",
< author = "Peng Tan and Wei Kong and Zongping Shao and Meilin Liu and Meng Ni",
< keywords = "Li air battery",
< keywords = "Modeling",
< keywords = "Working behavior",
< keywords = "Mechanism",
< keywords = "Challenges"
< }
462c437
< journal = {ACS Applied Materials \& Interfaces},
---
> journal = {ACS App. Mater. \& Inter.},
465c440
< pages = {4039-4047},
---
> pages = {4039--4047},
468,470d442
< note ={PMID: 25625507},
< URL = {http://dx.doi.org/10.1021/am5083254},
< eprint = {        http://dx.doi.org/10.1021/am5083254}
474,475c446,447
< author = {Luntz and V. Viswanathan and J. Voss and J. B. Varley and J. K. Norskov and R. Scheffler and A. Speideli},
< journal = {The Journal of Physical Chemistry Letters},
---
> author = {Luntz, Alan C. and Viswanathan, V. and Voss, J. and  Varley, J. B. and Norskov, J. K.  and  Scheffler, R.  and Speideli, A.},
> journal = {J. Phys Chem. Lett.},
478c450
< pages = {3494-3499},
---
> pages = {3494--3499},
481,482d452
< URL = {http://dx.doi.org/10.1021/jz401926f},
< eprint = {http://dx.doi.org/10.1021/jz401926f}
492,493c462
< pages  ="720-727",
< publisher  ="The Royal Society of Chemistry",
---
> pages  ="720--727",
495,496d463
< url  ="http://dx.doi.org/10.1039/C3EE42446D",
< abstract  ="It is now well accepted that charge transport through Li2O2 is a serious limitation in Li-O2 batteries. We report formation energies for the different charge states of Li{,} O and O2 vacancies in Li2O2 that could have important implications for charge transport through Li2O2. Charge transition levels are given as a function of the location of the Fermi level in Li2O2 relative to the valence band maximum (VBM). We argue that in Li-O2 discharge/charge electrochemistry{,} the Fermi level is pinned by LiO2 interface states at [similar]0.35 eV above the VBM and this causes the vacancies to be in positively charged states (weakly violating local charge neutrality). We show by non-equilibrium Greens function calculations of charge transport through a Au|Li2O2 + VLiq |Au metal-insulator-metal structure (with VLiq a Li vacancy of charge state q){,} that the +1 and 0 charge state induces considerable scattering for tunneling holes. This tunneling is the previously proposed dominant mechanism of charge transport in Li-O2 batteries at practical current densities at room temperature{,} although we also proposed a contribution from hole polaron migration at very low currents and higher temperatures. We suggest that scattering of the tunneling holes by the positively charged vacancies (and possibly hole polarons) is the origin of the resistive loss observed in Li-O2 discharges in bulk electrolysis cells (where other forms of resistance are negligible). Thus{,} we argue that charged vacancies hinder charge transport through Li2O2 in Li-O2 electrochemical discharges."}
506,507c473
< pages  ="2739-2752",
< publisher  ="The Royal Society of Chemistry",
---
> pages  ="2739--2752",
509,510d474
< url  ="http://dx.doi.org/10.1039/C4EE00496E",
< abstract  ="Understanding charge carrier transport in Li2O2{,} the storage material in the non-aqueous Li-O2 battery{,} is key to the development of this high-energy battery. Here{,} we studied ionic transport properties and Li self-diffusion in nanocrystalline Li2O2 by conductivity and temperature variable 7Li NMR spectroscopy. Nanostructured Li2O2{,} characterized by a mean crystallite size of less than 50 nm as estimated from X-ray diffraction peak broadening{,} was prepared by high-energy ball milling of microcrystalline lithium peroxide with [small mu ]m sized crystallites. At room temperature the overall conductivity [sigma] of the microcrystalline reference sample turned out to be very low (3.4 [times] 10-13 S cm-1) which is in agreement with results from temperature-variable 7Li NMR line shape measurements. Ball-milling{,} however{,} leads to an increase of [sigma] by approximately two orders of magnitude (1.1 [times] 10-10 S cm-1); correspondingly{,} the activation energy decreases from 0.89 eV to 0.82 eV. The electronic contribution [sigma]eon{,} however{,} is in the order of 9 [times] 10-12 S cm-1 which makes less than 10% of the total value. Interestingly{,} 7Li NMR lines of nano-Li2O2 undergo pronounced heterogeneous motional narrowing which manifests in a two-component line shape emerging with increasing temperatures. Most likely{,} the enhancement in [sigma] can be traced back to the generation of a spin reservoir with highly mobile Li ions; these are expected to reside in the nearest neighbourhood of defects generated or near the structurally disordered and defect-rich interfacial regions formed during mechanical treatment."}
520d483
<   numpages = {0},
522,523d484
<   month = {Feb},
<   publisher = {American Physical Society},
525d485
<   url = {https://link.aps.org/doi/10.1103/PhysRevB.51.4014}
531c491
< journal = {Journal of the American Chemical Society},
---
> journal = {J. Am. Chem. Soc.},
534c494
< pages = {16335-16344},
---
> pages = {16335--16344},
537,539d496
< note ={PMID: 25341076},
< URL = {http://dx.doi.org/10.1021/ja508794r},
< eprint = { http://dx.doi.org/10.1021/ja508794r}
542,572c499,508
< @article{PBE,
<   title = {Generalized Gradient Approximation Made Simple},
<   author = {Perdew, John P. and Burke, Kieron and Ernzerhof, Matthias},
<   journal = {Phys. Rev. Lett.},
<   volume = {77},
<   issue = {18},
<   pages = {3865--3868},
<   numpages = {0},
<   year = {1996},
<   month = {Oct},
<   publisher = {American Physical Society},
<   doi = {10.1103/PhysRevLett.77.3865},
<   url = {https://link.aps.org/doi/10.1103/PhysRevLett.77.3865}
< }
< 
< @misc{note1,
< note= prueba,
< }
< 
< @Article{li20,
< author ="Strange, J. H. and Rageb, S. M. and Chadwick, A. V. and Flack, K. W. and Harding, J. H.",
< title  ="Conductivity and NMR study of ionic mobility in lithium oxide",
< journal  ="J. Chem. Soc.{,} Faraday Trans.",
< year  ="1990",
< volume  ="86",
< issue  ="8",
< pages  ="1239-1241",
< publisher  ="The Royal Society of Chemistry",
< doi  ="10.1039/FT9908601239",
< url  ="http://dx.doi.org/10.1039/FT9908601239",
< abstract  ="The self-diffusion of Li ions in the ionic conductor LiO has been investigaed by Li NMR relaxation time and A.C. conductivity measurements. The NMR relaxation data have been fitted using an encounter model in order to obtain the mean jump time () and thence the diffusion coefficient of Li ions [eqn (1)]. We have established that the mobile ions are Li and that the mechanism for their diffusion is most probably cation vacancies."
---
> @article{TAN2017155,
> title = "Advances in modeling and simulation of Li air batteries",
> journal = "Progr. Energy Combust. Sci.",
> volume = "62",
> number = "Supplement C",
> pages = "155--189",
> year = "2017",
> issn = "0360-1285",
> doi = "https://doi.org/10.1016/j.pecs.2017.06.001",
> author = "Peng Tan and Wei Kong and Zongping Shao and Meilin Liu and Meng Ni",
576,600d511
< @article{Cota-2005,
< author = "Cota, Luis Guillermo and de la Mora, Pablo",
< title = "{On the structure of lithium peroxide, Li${\sb 2}$O${\sb 2}$}",
< journal = "Acta Crystallographica Section B",
< year = "2005",
< volume = "61",
< number = "2",
< pages = "133--136",
< month = "Apr",
< doi = {10.1107/S0108768105003629},
< url = {https://doi.org/10.1107/S0108768105003629},
< abstract = {The two published lithium peroxide structures, both ascribed to the hexagonal P\bar 6 space group, were subjected to reinterpretation, and another more symmetric structure, now belonging to the {\it P}6${\sb 3}$/{\it mmc} space group, was found. Detailed density-functional quantum mechanical calculations and crystal structure optimizations were carried out on both structures and the energetic arguments obtained therewith helped to rule out one of them.},
< keywords = {crystal structure optimization, quantum-mechanical calculations},
< }
< 
< @article{Chan-2011,
< author = {Chan, Maria K. Y. and Shirley, Eric L. and Karan, Naba K. and Balasubramanian, Mahalingam and Ren, Yang and Greeley, Jeffrey P. and Fister, Tim T.},
< title = {Structure of Lithium Peroxide},
< journal = {The Journal of Physical Chemistry Letters},
< volume = {2},
< number = {19},
< pages = {2483-2486},
< year = {2011},
< doi = {10.1021/jz201072b},
< }

